CS-Insights: A System for Analyzing Computer Science Research

This paper presents CS-Insights, an interactive web application to analyze computer science publications from DBLP through multiple perspectives. The dedicated interfaces allow its users to identify trends in research activity, productivity, accessibility, author's productivity, venues' statistics, topics of interest, and the impact of computer science research on other fields. CS-Insightsis publicly available, and its modular architecture can be easily adapted to domains other than computer science.

==> tables/ap_comm_acm_comparison.tex <==
% Table generated by Excel2LaTeX from sheet 'ACM topics'
\begin{table}[htbp]
  \centering
  \caption{Comparison of the most salient terms for the Communication of ACM venue in 1999, 2009 and 2019.}
    \begin{tabular}{lll}
    \toprule
    \multicolumn{1}{r}{\textbf{1999}} & \multicolumn{1}{r}{\textbf{2009}} & \multicolumn{1}{r}{\textbf{2019}} \\
    \midrule
    test  & web   & cacm \\
    agent & secur & comput \\
    email & journal & blog \\
    usabl & softwar & http \\
    fax   & commun & twitter \\
    data  & comput & corpor \\
    digit & system & commun \\
    design & project & acm \\
    network & scienc & org \\
    virtual & inform & algorithm \\
    softwar & adopt & technolog \\
    isd   & team  & softwar \\
    real  & virtual & web \\
    emerg & acm   & quantum \\
    internet & technolog & machin \\
    engin & custom & quic \\
    inform & publish & system \\
    product & manag & industri \\
    system & develop & research \\
    user  & privaci & india \\
    qualiti & citat & predict \\
    comput & internet & scienc \\
    knowledg & parallel & data \\
    world & nativ & protocol \\
    applic & translat & inform \\
    student & site  & languag \\
    develop & firm  & learn \\
    realiti & item  & indian \\
    engel & american & right \\
    andrzejewski & servic & servic \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> tables/field_influence.tex <==
% Table generated by Excel2LaTeX from sheet 'Q1_A_Latex'
\begin{table}[htbp]
  \centering
  \small
  \caption{Computer science venue overlap with other fields for top-100 venues wrt \#papers and \#citations. Intra-field shows how much venue overlap each field has for \#papers and \#citations }
    \begin{tabular}{lrrr}
    \toprule
    \textbf{Field}      & \textbf{Intra-field (\%)} & \textbf{Papers (\%)} & \textbf{Citations (\%)} \\
    \midrule
    CS    & 54    & 54    & 54 \\
    MT    & 64    & 47    & 55 \\
    EN    & 68    & 28    & 22 \\
    MD    & 84    & 14    & 22 \\
    PS    & 66    & 14    & 16 \\
    \bottomrule
    \end{tabular}%
  \label{tab:field_influence}%
\end{table}%


==> tables/venues_authors_stats.tex <==
% Table generated by Excel2LaTeX from sheet 'Q2_Bb_latex'
\begin{table}[htbp]
  \centering
  \small
  \caption{Common venues published by top-5 authors wrt their \#papers and \#citations}
    \begin{tabular}{rllr}
    \toprule
    \multicolumn{4}{c}{\textbf{Paper}} \\
    \multicolumn{1}{l}{\textbf{\#Papers}} & \multicolumn{1}{c}{\textbf{Venue}} & \multicolumn{1}{c}{\textbf{Area}} & \multicolumn{1}{l}{\textbf{h-ind}} \\
    \midrule
    22296 & ICC   & Net. and com. & 75 \\
    16325 & IT. Inf. Theory & Inf. theory & \textbf{279} \\
    15395 & IT. Com. & Sig. proc. & 216 \\
    13328 & IT. Signal Process. & Sig. proc. & 275 \\
    11683 & IT. Veh. Technol. & Vehicles & 188 \\
    9372  & IT. Wirel. Com. & Sig. proc. & 224 \\
    4385  & KDD   & DBM & 114 \\
    4277  & IT. Knowl. Data Eng. & DBM & 183 \\
    3312  & ICDM  & DBM & \textit{53} \\
    \midrule
    \multicolumn{4}{c}{\textbf{Citation}} \\
    \multicolumn{1}{l}{\textbf{\#Citations}} & \multicolumn{1}{c}{\textbf{Venue}} & \multicolumn{1}{c}{\textbf{Area}} & \multicolumn{1}{l}{\textbf{h-ind}} \\
    \midrule
    1621492 & CVPR  & CV & \textbf{389} \\
    1337060 & IT. PA. M. Int. & CV & 377 \\
    601139 & ICCV  & CV & 239 \\
    495433 & ECCV  & CV & 186 \\
    328734 & AT. Graph. & CV & 221 \\
    263301 & Int. J. Comp. Vis. & CV & 201 \\
    191719 & ICPR  & Pat. recog. & 110 \\
    185792 & A. Multimedia & Multimedia & \textit{70} \\
    126888 & IT. Inf. For. Sec. & Security & 140 \\
    91693 & BMVC  & CV & 75 \\
    \bottomrule
    \end{tabular}%
  \label{tab:venues_authors_stats}%
\end{table}%


==> tables/venues_stats.tex <==
% Table generated by Excel2LaTeX from sheet 'Q2_Bb_latex'
\begin{table}[htbp]
  \centering
  \small
  \caption{Overall top-10 venues wrt their \#papers and \#citations}
    \begin{tabular}{rllr}
    \toprule
    \multicolumn{4}{c}{\textbf{Paper}} \\
    \multicolumn{1}{l}{\textbf{\#Papers}} & \multicolumn{1}{c}{\textbf{Venue}} & \multicolumn{1}{c}{\textbf{Area}} & \multicolumn{1}{l}{\textbf{h-ind}} \\
    \midrule
    54961 & I. Access & Misc  &\textbf{ 158} \\
    45660 & ICASSP & Sig. proc. & 110 \\
    36718 & Sensors & Sig. proc & 145 \\
    29421 & IGARSS & Sig. proc & 41 \\
    25017 & ICRA  & Aut. and rob. & 116 \\
    23549 & ISCAS & Hardware & \textit{38} \\
    22714 & ICIP  & CV & 88 \\
    22296 & ICC   & Net and com. & 75 \\
    19983 & Ap. Ma. Comp. & Mathematics & 154 \\
    19561 & IROS  & Aut. and rob. & 80 \\
    \midrule
    \multicolumn{4}{c}{\textbf{Citation}} \\
    \multicolumn{1}{l}{\textbf{\#Citations}} & \multicolumn{1}{c}{\textbf{Venue}} & \multicolumn{1}{c}{\textbf{Area}} & \multicolumn{1}{l}{\textbf{h-ind}} \\
    \midrule
    1621492 & CVPR  & CV & \textbf{389} \\
    1377202 & NeuroImage & Neuroscience & 381 \\
    1337060 & IT. PA. M. Int. & CV & 377 \\
    1147862 & IT. Inf. Theory & Inf. Theory & 279 \\
    946576 & Com. ACM & Misc  & 220 \\
    802571 & IT. Ind. Elec. & App. and Eng. & 304 \\
    790170 & ICRA  & Aut. and rob. & 116 \\
    762802 & IT. Sig. Proc. & Sig. proc & 275 \\
    717910 & IT. Aut. Cont. & Aut. and rob. & 300 \\
    714945 & ICASSP & Sig. proc & \textit{110} \\
    \bottomrule
    \end{tabular}%
  \label{tab:venues_overall_stats}%
\end{table}%

